Will It Go Viral? Grounding Micro-Video Popularity Prediction on the Open Web

Micro-video popularity prediction (MVPP) forecasts the popularity a newly uploaded short-form video will attract within a fixed number of days after upload. This task supports downstream applications in recommendation, advertising, and creator analytics, yet the problem is hard since virality depends on external trends rather than video content alone. Prior MVPP methods incorporate context by retrieving similar videos from platform-internal corpora, however historical neighbors cannot reveal whether a topic is currently trending, controversial, or already saturated across the open web. To this end, we reformulate MVPP as open-web grounded prediction and introduce WEBSHORTS, the first micro-video dataset that couples 14K videos with real-time open-web context collected at upload time, alongside daily view counts tracked over 7 days. The context for each video is organized as a structured evidence-card that captures the external attention landscape along three complementary web-context dimensions. We further propose SHORTS-CAST, a framework that generates dimension-wise rationales from the evidence-card to guide popularity regression, then adapts at deployment by selectively updating the context-to-popularity mapping when delayed labels reveal genuine trend shifts. In our experiments, SHORTS-CAST consistently outperforms content-only, video corpus retrieval-augmented, and online adaptation baselines under both offline and delayed-label online protocols, confirming that structured web context and trend-aware adaptation are jointly necessary for popularity forecasting under realistic deployment constraints in fast-evolving short-form video ecosystems.

==> TAB/062_prior_methods_w_web.tex <==
% preamble: \usepackage{wrapfig}

% \begin{wraptable}{l}{0.5\columnwidth}
% % \vspace{-0.3cm}  % 문단 상단과 높이 맞춤
% \centering
% \scriptsize
% \setlength{\tabcolsep}{2pt}
% \renewcommand{\arraystretch}{1.05}
% \begin{tabular}{lccc}
% \toprule
% & \textbf{nMSE} ($\downarrow$) & \textbf{MAE} ($\downarrow$) & \textbf{SRC} ($\uparrow$) \\
% \midrule
% MMRA & 0.807 & 2.915 & 0.480 \\
% \rowcolor{black!7}\textbf{+ Evidence Card} & \textbf{0.786} & \textbf{2.840} & \textbf{0.494} \\
% \midrule
% ICPF & 0.794 & 2.817 & 0.478 \\
% \rowcolor{black!7}\textbf{+ Evidence Card} & \textbf{0.787} & \textbf{2.807} & \textbf{0.489} \\
% \midrule
% EvoPro & 0.822 & 2.894 & 0.458 \\
% \rowcolor{black!7}\textbf{+ Evidence Card} & \textbf{0.816} & \textbf{2.872} & \textbf{0.466} \\
% \bottomrule
% \end{tabular}
% \caption{TEMP}
% \label{tab:prior_methods}
% \end{wraptable}

% ################################################################################

\begin{wraptable}{l}{0.5\columnwidth}
% \vspace{-0.3cm} 
\caption{Performance comparison of prior methods with and w/o evidence-card augmentation}
\centering
\scriptsize
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{lcccc}
\toprule
\textbf{Method} & \textbf{nMSE} ($\downarrow$) & \textbf{MAE} ($\downarrow$) & \textbf{SRC} ($\uparrow$) & \textbf{PCC} ($\uparrow$) \\
\midrule
MMRA~\cite{zhong2024mmra} & 0.807 & 2.915 & 0.480 & 0.458 \\
\rowcolor{black!7}\textbf{+ Evidence-Card} & \textbf{0.786} & \textbf{2.840} & \textbf{0.494} & \textbf{0.470} \\
\midrule
ICPF~\cite{cheng2025incontext} & 0.794 & 2.817 & 0.478 & 0.454 \\
\rowcolor{black!7}\textbf{+ Evidence-Card} & \textbf{0.787} & \textbf{2.807} & \textbf{0.489} & \textbf{0.462} \\
\midrule
EvoPro~\cite{chen2025echoes} & 0.822 & 2.894 & 0.458 & 0.425 \\
\rowcolor{black!7}\textbf{+ Evidence-Card} & \textbf{0.816} & \textbf{2.872} & \textbf{0.466} & \textbf{0.432} \\
\midrule
\proposed (\textit{Offline}) & \textbf{0.701} & \textbf{2.453} & \textbf{0.612} & \textbf{0.594} \\
\bottomrule
\end{tabular}
\label{tab:prior_methods}
\end{wraptable}


% \begin{wraptable}{l}{0.5\columnwidth}
% % \vspace{-0.3cm} 
% \caption{Performance comparison of prior methods with and w/o evidence-card augmentation}
% \centering
% \scriptsize
% \setlength{\tabcolsep}{2pt}
% \renewcommand{\arraystretch}{1.05}
% \begin{tabular}{lcccc}
% \toprule
% \textbf{Method} & \textbf{nMSE} ($\downarrow$) & \textbf{MAE} ($\downarrow$) & \textbf{SRC} ($\uparrow$) & \textbf{PCC} ($\uparrow$) \\
% \midrule
% MMRA~\cite{zhong2024mmra} & 0.807 & 2.915 & 0.480 & 0.458 \\
% \rowcolor{black!7}\textbf{+ Evidence-Card} & \textbf{0.786} & \textbf{2.840} & \textbf{0.494} & \textbf{0.470} \\
% \midrule
% ICPF~\cite{cheng2025incontext} & 0.794 & 2.817 & 0.478 & 0.454 \\
% \rowcolor{black!7}\textbf{+ Evidence-Card} & \textbf{0.787} & \textbf{2.807} & \textbf{0.489} & \textbf{0.462} \\
% \midrule
% EvoPro~\cite{chen2025echoes} & 0.822 & 2.894 & 0.458 & 0.425 \\
% \rowcolor{black!7}\textbf{+ Evidence-Card} & \textbf{0.816} & \textbf{2.872} & \textbf{0.466} & \textbf{0.432} \\
% \bottomrule
% \end{tabular}
% \label{tab:prior_methods}
% \end{wraptable}

% \begin{table}[t]
% \caption{Performance comparison of prior methods with and without evidence card augmentation.}
% \centering
% \scriptsize
% \setlength{\tabcolsep}{3pt}
% \renewcommand{\arraystretch}{1.05}
% \begin{tabular}{lcccc}
% \toprule
% \textbf{Method} & \textbf{nMSE} ($\downarrow$) & \textbf{MAE} ($\downarrow$) & \textbf{SRC} ($\uparrow$) & \textbf{PCC} ($\uparrow$) \\
% \midrule
% MMRA~\cite{zhong2024mmra} & 0.807 & 2.915 & 0.480 & 0.458 \\
% \rowcolor{black!7}\textbf{+ Evidence Card} & \textbf{0.786} & \textbf{2.840} & \textbf{0.494} & \textbf{0.470} \\
% \midrule
% ICPF~\cite{cheng2025incontext} & 0.794 & 2.817 & 0.478 & 0.454 \\
% \rowcolor{black!7}\textbf{+ Evidence Card} & \textbf{0.787} & \textbf{2.807} & \textbf{0.489} & \textbf{0.462} \\
% \midrule
% EvoPro~\cite{chen2025echoes} & 0.822 & 2.894 & 0.458 & 0.425 \\
% \rowcolor{black!7}\textbf{+ Evidence Card} & \textbf{0.816} & \textbf{2.872} & \textbf{0.466} & \textbf{0.432} \\
% \bottomrule
% \end{tabular}
% \label{tab:prior_methods}
% \end{table}
